Secondary eclipse observations for seven hot-Jupiters from the Anglo-Australian Telescope

We report detections and constraints for the near infrared Ks band secondary eclipses of seven hot-Jupiters using the IRIS2 infrared camera on the Anglo-Australian Telescope. Eclipses in the Ks band for WASP-18b and WASP-36b have been measured for the first time. We also present new measurements for the eclipses of WASP-4b, WASP-5b, and WASP-46b, as well as upper limits for the eclipse depths of WASP-2b and WASP-76b. In particular, two full eclipses of WASP-46b were observed, allowing us to demonstrate the repeatability of our observations via independent analyses on each eclipse. Significant numbers of eclipse depths for hot-Jupiters have now been measured in both Ks and the four Spitzer IRAC bandpasses. We discuss these measurements in the context of the broadband colours and brightness temperatures of the hot-Jupiter atmosphere distribution. Specifically, we re-examine the proposed temperature dichotomy between the most irradiated, and mildly irradiated planets. We find no evidence for multiple clusters in the brightness temperature - equilibrium temperature distributions in any of these bandpasses, suggesting a continuous distribution of heat re-emission and circulation characteristics for these planets.

==> BD_refs.tex <==
\onecolumn
{\footnotesize \begin{longtable}{lp{10cm}}

\caption{Primary references for brown dwarf parallaxes and photometry } \label{tab:BD_ref}\\

\hline\hline Brown dwarf & \multicolumn{1}{l}{References} \\ \hline 
\endfirsthead

\multicolumn{2}{c}%
{ \tablename\ \thetable{} -- continued from previous page} \\
\hline\hline Brown dwarf & \multicolumn{1}{l}{References} \\ \hline 
\endhead

\hline \multicolumn{2}{r}{{Continued on next page}} \\ \hline
\endfoot

\hline
\endlastfoot

{2MASSIJ0003422-282241} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{GJ1001B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002MNRAS.332...78L,2006AJ....132.2360H,2006ApJ...651..502P}} \\ 
{GJ1001C} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002MNRAS.332...78L,2006AJ....132.2360H,2006ApJ...651..502P}} \\ 
{LSRJ0011+5908} & {\citet{2003tmc..book.....C,2009AJ....137.4109L,2010AJ....140.1868W}} \\ 
{HD1160B} & {\citet{2012ApJ...750...53N,2007ASSL..350.....V}} \\ 
{LHS1070A} & {\citet{2012ApJS..201...19D,1998ApJ...509..836L,2003tmc..book.....C,2005AJ....130..337C}} \\ 
{LHS1070B} & {\citet{2012ApJS..201...19D,1998ApJ...509..836L,2003tmc..book.....C,2005AJ....130..337C}} \\ 
{LHS1070C} & {\citet{2012ApJS..201...19D,1998ApJ...509..836L,2003tmc..book.....C,2005AJ....130..337C}} \\ 
{2MASSJ00250365+4759191A} & {\citet{2003tmc..book.....C,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{2MASSJ00250365+4759191B} & {\citet{2003tmc..book.....C,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{PC0025+0447} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{2MASSWJ0030300-145033} & {\citet{2012ApJS..201...19D,2004AJ....127.2948V,2004AJ....127.3553K,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{SDSSpJ003259.36+141036.6} & {\citet{2004AJ....127.2948V,2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2004AJ....127.3516G}} \\ 
{RG0050-2722} & {\citet{1996MNRAS.281..644T,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{CFBDSJ005910.90-011401.3} & {\citet{2012ApJS..201...19D,2008A&A...482..961D,2010AJ....140.1868W}} \\ 
{SDSSpJ010752.33+004156.1} & {\citet{2012ApJS..201...19D,2004AJ....127.2948V,2002ApJ...564..452L,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{CTI012657.5+280202} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{L726-8A} & {\citet{1988AJ.....95.1841G,2003tmc..book.....C,1993AJ....106..773H,2010AJ....140.1868W}} \\ 
{L726-8B} & {\citet{1988AJ.....95.1841G,2003tmc..book.....C,1993AJ....106..773H,2010AJ....140.1868W}} \\ 
{2MASSJ01490895+2956131} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{GJ1048B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2007ASSL..350.....V}} \\ 
{BRIB0246-1703} & {\citet{1996MNRAS.281..644T,2003tmc..book.....C,1998ApJ...509..836L,2010AJ....140.1868W}} \\ 
{TVLM831-154910} & {\citet{2003tmc..book.....C,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{TVLM831-161058} & {\citet{2003tmc..book.....C,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{TVLM831-165166} & {\citet{2003tmc..book.....C,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{TVLM832-10443} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{PSOJ043.5395+02.3995} & {\citet{2011ApJ...740L..32L,2010AJ....140.1868W}} \\ 
{TVLM832-42500} & {\citet{2003tmc..book.....C,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{LP412-31} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{2MASSWJ0326137+295015} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{2MASSIJ0328426+230205} & {\citet{2004AJ....127.2948V,2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2004AJ....127.3516G}} \\ 
{LSPMJ0330+5413} & {\citet{2003tmc..book.....C,2009AJ....137.4109L,2010AJ....140.1868W}} \\ 
{2MASPJ0345432+254023} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W,2001ApJ...548..908L,2002ApJ...564..452L}} \\ 
{LHS1604} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1998ApJ...509..836L,1992AJ....103..638M}} \\ 
{SDSSpJ042348.57-041403.5B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2004AJ....127.3516G,2006ApJ...651..502P}} \\ 
{LHS191} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1992AJ....103..638M}} \\ 
{LHS197} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1992AJ....103..638M}} \\ 
{LSRJ0510+2713} & {\citet{2003tmc..book.....C,2009AJ....137.4109L,2010AJ....140.1868W}} \\ 
{LSRJ0515+5911} & {\citet{2003tmc..book.....C,2009AJ....137.4109L,2010AJ....140.1868W}} \\ 
{2MASSJ05185995-2828372B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{LHS207} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1992AJ....103..638M}} \\ 
{{beta}Pic~b} & {\citet{2011A&A...528L..15B,2011ApJ...736L..33C,2007ASSL..350.....V}} \\ 
{2MASSJ06411840-4322329} & {\citet{2011AJ....141...54A,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{ESO207-61} & {\citet{1996MNRAS.281..644T,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{2MASSJ07193188-5051410} & {\citet{2011AJ....141...54A,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{LHS234} & {\citet{1998ApJ...509..836L,2003tmc..book.....C,2005AJ....130..337C,2010AJ....140.1868W}} \\ 
{2MASSIJ0746425+200032A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2010ApJ...711.1087K,2006ApJ...651..502P}} \\ 
{2MASSIJ0746425+200032B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2010ApJ...711.1087K,2006ApJ...651..502P}} \\ 
{LP423-31} & {\citet{2003tmc..book.....C,2009AJ....137..402G,2010AJ....140.1868W}} \\ 
{HD65216B} & {\citet{2007MNRAS.378.1328M,2007ASSL..350.....V}} \\ 
{HD65216C} & {\citet{2007MNRAS.378.1328M,2007ASSL..350.....V}} \\ 
{HIP38939B} & {\citet{2012ApJ...755...94D,2003tmc..book.....C,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{SDSSJ080531.84+481233.0B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2007ApJ...655.1079L,2004AJ....127.3553K,2004AJ....127.3516G}} \\ 
{WD0806-661B} & {\citet{2012ApJ...744..135L,2009AJ....137.4547S,2010AJ....140.1868W}} \\ 
{DENISJ081730.0-615520} & {\citet{2003tmc..book.....C,2010ApJ...718L..38A,2010AJ....140.1868W}} \\ 
{ULASJ082707.67-020408.2} & {\citet{2007MNRAS.379.1423L,2010A&A...524A..38M}} \\ 
{LHS248} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1995gcts.book.....V,2006ApJ...651..502P}} \\ 
{SDSSpJ083008.12+482847.4} & {\citet{2004AJ....127.2948V,2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2007ApJ...655.1079L}} \\ 
{LHS2021} & {\citet{2010AJ....140.1868W,2003tmc..book.....C,2006AJ....132.1234C,2006ApJ...651..502P}} \\ 
{LHS2026} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1992AJ....103..638M}} \\ 
{2MASSJ08354256-0819237} & {\citet{2012ApJS..201...19D,2011AJ....141...54A,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{LHS2034} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1992AJ....103..638M}} \\ 
{2MASSIJ0856479+223518A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{2MASSIJ0856479+223518B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{LP368-128} & {\citet{2006AJ....132.2360H,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{ULASJ090116.23-030635.0} & {\citet{2007MNRAS.379.1423L,2010A&A...524A..38M,2010AJ....140.1868W}} \\ 
{DENIS-PJ0909.9-0658} & {\citet{2011AJ....141...54A,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{TVLM262-111511} & {\citet{2003tmc..book.....C,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{ULASJ094806.06+064805.0} & {\citet{2007MNRAS.379.1423L,2010A&A...524A..38M}} \\ 
{LP261-75B} & {\citet{2004AJ....127.2948V,2003tmc..book.....C}} \\ 
{TVLM262-70502} & {\citet{2003tmc..book.....C,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{2MASSJ09522188-1924319A} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{2MASSJ09522188-1924319B} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{2MASSJ10043929-3335189} & {\citet{2011AJ....141...54A,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{TVLM263-71765} & {\citet{2003tmc..book.....C,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{ULASJ101821.78+072547.1} & {\citet{2007MNRAS.379.1423L,2010A&A...524A..38M}} \\ 
{2MASSJ10185879-2909535} & {\citet{2011AJ....141...54A,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{SDSSJ102109.69-030420.1B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2000ApJ...536L..35L,2004AJ....127.3516G,2006ApJ...651..502P}} \\ 
{TVLM213-2005} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{HD89744B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{LHS2314} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1998ApJ...509..836L,1992AJ....103..638M}} \\ 
{Wolf359} & {\citet{1995gcts.book.....V,2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2002AJ....123.2806R}} \\ 
{SSSPMJ1102-3431} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2008A&A...489..825T,2010AJ....140.1868W}} \\ 
{LHS2351} & {\citet{1996MNRAS.281..644T,2003tmc..book.....C,1998ApJ...509..836L,2010AJ....140.1868W}} \\ 
{LHS2397aA} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2002ApJ...564..452L,2009ApJ...699..168D,2010AJ....140.1868W}} \\ 
{LHS2397aB} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2002ApJ...564..452L,2009ApJ...699..168D,2010AJ....140.1868W}} \\ 
{ULASJ115038.79+094942.9} & {\citet{2010A&A...524A..38M,2008MNRAS.390..304P}} \\ 
{LHS2471} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1992AJ....103..638M}} \\ 
{2MASSWJ1200329+204851} & {\citet{2003tmc..book.....C,1995gcts.book.....V,2010AJ....140.1868W}} \\ 
{2MASSJ12095613-1004008A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010ApJ...722..311L,2010AJ....140.1868W,2006AJ....131.2722C}} \\ 
{BRIB1222-1222} & {\citet{1996MNRAS.281..644T,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{2MASSJ12255432-2739466A} & {\citet{2003AJ....126..975T,2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2006ApJ...651..502P}} \\ 
{2MASSJ12255432-2739466B} & {\citet{2003AJ....126..975T,2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2006ApJ...651..502P}} \\ 
{LHS330} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1998ApJ...509..836L,1992AJ....103..638M}} \\ 
{2MASSWJ1239272+551537A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{2MASSWJ1239272+551537B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{SSSPMJ1256-1408} & {\citet{2003tmc..book.....C,2009A&A...493L..27S,2010AJ....140.1868W}} \\ 
{Ross458C} & {\citet{2010MNRAS.405.1140G,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{ULASJ131508.42+082627.4} & {\citet{2010A&A...524A..38M,2008MNRAS.390..304P}} \\ 
{2MASSJ13204159+0957506} & {\citet{2003tmc..book.....C,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{2MASSWJ1328550+211449} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{2MASSJ14044948-3159330B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{GD165B} & {\citet{1995gcts.book.....V,2003tmc..book.....C,2010AJ....140.1868W,2002ApJ...564..452L,2006MNRAS.367..454H,1996MNRAS.280...77J}} \\ 
{LHS2919} & {\citet{2003tmc..book.....C,2009AJ....137.4109L,2010AJ....140.1868W}} \\ 
{ProximaCen} & {\citet{2003tmc..book.....C,1999AJ....118.1086B,2010AJ....140.1868W}} \\ 
{LHS2930} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1992AJ....103..638M}} \\ 
{SDSSJ143517.20-004612.9} & {\citet{2004AJ....127.2948V,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{SDSSJ143535.72-004347.0} & {\citet{2004AJ....127.2948V,2004AJ....127.3553K,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{DENIS-PJ144137.3-094559A} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{DENIS-PJ144137.3-094559B} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{SDSSpJ144600.60+002452.0} & {\citet{2004AJ....127.2948V,2002ApJ...564..452L,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{Gl569Ba} & {\citet{2007ASSL..350.....V,2012ApJS..201...19D,2010ApJ...721.1725D,2001ApJ...560..390L,1988ApJ...330L.119F}} \\ 
{Gl569Bb} & {\citet{2007ASSL..350.....V,2012ApJS..201...19D,2010ApJ...721.1725D,2001ApJ...560..390L,1988ApJ...330L.119F}} \\ 
{CFBDSJ145829+10134A} & {\citet{2012ApJS..201...19D,2012yCat.2310....0U,2010AJ....140.1868W,2011ApJ...740..108L,2010A&A...518A..39D}} \\ 
{TVLM513-46546} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,1998ApJ...509..836L,2002ApJ...564..452L,2010AJ....140.1868W}} \\ 
{TVLM513-42404} & {\citet{2003tmc..book.....C,1998ApJ...509..836L,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{TVLM513-42404B} & {\citet{2003tmc..book.....C,1998ApJ...509..836L,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{2MASSWJ1503196+252519} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2007ApJ...655.1079L,2004AJ....127.3553K,2004AJ....127.3516G}} \\ 
{TVLM868-110639} & {\citet{2003tmc..book.....C,1998ApJ...509..836L,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{TVLM513-8328} & {\citet{2003tmc..book.....C,1998ApJ...509..836L,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{Gl584C} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2002ApJ...564..452L,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{SDSSJ153417.05+161546.1B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2006ApJ...647.1393L,2010AJ....140.1868W,2006AJ....131.2722C}} \\ 
{2MASSIJ1534498-295227A} & {\citet{2008ApJ...689..436L,2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2004AJ....127.3553K,2004AJ....127.3516G,2006ApJ...651..502P}} \\ 
{2MASSIJ1534498-295227B} & {\citet{2008ApJ...689..436L,2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2004AJ....127.3553K,2004AJ....127.3516G,2006ApJ...651..502P}} \\ 
{WISEPAJ154151.66-225025.2} & {\citet{2011ApJS..197...19K,2010AJ....140.1868W}} \\ 
{2MASSJ15462718-3325111} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2003AJ....126..975T,2010AJ....140.1868W}} \\ 
{2MASSWJ1553022+153236A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2007ApJ...655.1079L,2004AJ....127.3553K,2006ApJ...651..502P}} \\ 
{2MASSWJ1553022+153236B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2007ApJ...655.1079L,2004AJ....127.3553K,2006ApJ...651..502P}} \\ 
{LSRJ1610-0040A} & {\citet{2008ApJ...686..548D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{LSRJ1610-0040B} & {\citet{2008ApJ...686..548D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{GJ618.1B} & {\citet{2003tmc..book.....C,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{LHS3241} & {\citet{2003tmc..book.....C,2009AJ....137..402G,2010AJ....140.1868W}} \\ 
{2MASSWJ1658037+702701} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{DENIS-PJ170548.3-051645} & {\citet{2012ApJS..201...19D,2011AJ....141...54A,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{2MASSIJ1711457+223204} & {\citet{2012ApJS..201...19D,2004AJ....127.2948V,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{GJ660.1B} & {\citet{2003tmc..book.....C,2007ASSL..350.....V}} \\ 
{LSPMJ1735+2634A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{WISEPJ174124.27+255319.6} & {\citet{2011ApJS..197...19K,2010AJ....140.1868W}} \\ 
{2MASSJ17502484-0016151} & {\citet{2012ApJS..201...19D,2011AJ....141...54A,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{LP44-162} & {\citet{2003tmc..book.....C,2009AJ....137.4109L,2010AJ....140.1868W}} \\ 
{SDSSJ175805.46+463311.9} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2004AJ....127.3553K,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{2MASSIJ1835379+325954} & {\citet{2003AJ....125..354R,2010AJ....140.1868W,2003tmc..book.....C,2006ApJ...651..502P}} \\ 
{LP335-12} & {\citet{2003tmc..book.....C,2009AJ....137.4109L,2010AJ....140.1868W}} \\ 
{LP44-334} & {\citet{2003tmc..book.....C,2009AJ....137.4109L,2010AJ....140.1868W}} \\ 
{CE507} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{LHS3406} & {\citet{2003tmc..book.....C,2010AJ....140.1868W,1998ApJ...509..836L,1992AJ....103..638M}} \\ 
{SCRJ1845-6357A} & {\citet{2006AJ....132.2360H,2003tmc..book.....C,2007A&A...471..655K,2010AJ....140.1868W}} \\ 
{SCRJ1845-6357B} & {\citet{2006AJ....132.2360H,2003tmc..book.....C,2007A&A...471..655K,2010AJ....140.1868W}} \\ 
{2MASSIJ1847034+552243A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010ApJ...711.1087K,2010AJ....140.1868W}} \\ 
{2MASSIJ1847034+552243B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010ApJ...711.1087K,2010AJ....140.1868W}} \\ 
{PZTel~B} & {\citet{2007ASSL..350.....V,2010ApJ...720L..82B}} \\ 
{HR7329B} & {\citet{2007ASSL..350.....V,2000ApJ...541..390L}} \\ 
{Gl758B} & {\citet{2007ASSL..350.....V,2011ApJ...728...85J}} \\ 
{GJ1245B} & {\citet{2003tmc..book.....C,1993AJ....105.1571H,2010AJ....140.1868W}} \\ 
{SDSSJ205235.31-160929.8B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010AJ....140.1868W,2006AJ....131.2722C}} \\ 
{LP397-10} & {\citet{2003tmc..book.....C,2009AJ....137..402G,2010AJ....140.1868W}} \\ 
{[HB88]M18} & {\citet{1996MNRAS.281..644T,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{HD203030B} & {\citet{2007ASSL..350.....V,2006ApJ...651.1166M}} \\ 
{LSPMJ2124+4003} & {\citet{2003tmc..book.....C,2009AJ....137..402G,2010AJ....140.1868W}} \\ 
{HB2124-4228} & {\citet{1996MNRAS.281..644T,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{[HB88]M20} & {\citet{1996MNRAS.281..644T,2003tmc..book.....C,2010AJ....140.1868W}} \\ 
{2MASSWJ2140293+162518A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010ApJ...711.1087K,2010AJ....140.1868W}} \\ 
{2MASSWJ2140293+162518B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2010ApJ...711.1087K,2010AJ....140.1868W}} \\ 
{LSPMJ2158+6117} & {\citet{2003tmc..book.....C,2009AJ....137..402G,2010AJ....140.1868W}} \\ 
{{epsilon}Ind~Ba} & {\citet{2010AJ....140.1868W,2003tmc..book.....C,2010A&A...510A..99K,2007ASSL..350.....V,2006ApJ...651..502P}} \\ 
{{epsilon}Ind~Bb} & {\citet{2010AJ....140.1868W,2003tmc..book.....C,2010A&A...510A..99K,2007ASSL..350.....V,2006ApJ...651..502P}} \\ 
{2MASSWJ2206228-204705A} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2009ApJ...706..328D,2010AJ....140.1868W}} \\ 
{2MASSWJ2206228-204705B} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2009ApJ...706..328D,2010AJ....140.1868W}} \\ 
{GRH2208-20} & {\citet{2003tmc..book.....C,2002AJ....124.1170D,2010AJ....140.1868W}} \\ 
{TVLM890-60235} & {\citet{2003tmc..book.....C,1995AJ....110.3014T,2010AJ....140.1868W}} \\ 
{LHS523} & {\citet{2003tmc..book.....C,1995gcts.book.....V,2010AJ....140.1868W}} \\ 
{LP460-44} & {\citet{2003tmc..book.....C,2009AJ....137..402G,2010AJ....140.1868W}} \\ 
{G216-7B} & {\citet{2003tmc..book.....C,2007ASSL..350.....V,2010AJ....140.1868W}} \\ 
{ULASJ223955.76+003252.6} & {\citet{2007MNRAS.379.1423L,2010A&A...524A..38M}} \\ 
{2MASSJ23062928-0502285} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{HR8799b} & {\citet{2011ApJ...739L..41G,2013A&A...549A..52E,2007ASSL..350.....V,2008Sci...322.1348M}} \\ 
{HR8799c} & {\citet{2011ApJ...739L..41G,2013A&A...549A..52E,2007ASSL..350.....V,2008Sci...322.1348M}} \\ 
{HR8799e} & {\citet{2013A&A...549A..52E,2010Natur.468.1080M,2007ASSL..350.....V}} \\ 
{HR8799d} & {\citet{2011ApJ...739L..41G,2013A&A...549A..52E,2007ASSL..350.....V,2008Sci...322.1348M}} \\ 
{APMPMJ2330-4737} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{2MASSJ23310161-0406193A} & {\citet{2003tmc..book.....C,2007ASSL..350.....V,2002ApJ...567L..53C,2010AJ....140.1868W}} \\ 
{2MASSJ23310161-0406193B} & {\citet{2003tmc..book.....C,2007ASSL..350.....V,2002ApJ...567L..53C,2010AJ....140.1868W}} \\ 
{APMPMJ2331-2750} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{APMPMJ2344-2906} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 
{APMPMJ2354-3316C} & {\citet{2012ApJS..201...19D,2003tmc..book.....C,2009AJ....137.4547S,2010AJ....140.1868W}} \\ 
{APMPMJ2359-6246} & {\citet{2003tmc..book.....C,2006AJ....132.1234C,2010AJ....140.1868W}} \\ 



\end{longtable}
}
\twocolumn

